Hate Speech Detection: A Solved Problem? The Challenging Case of Long Tail on Twitter

In recent years, the increasing propagation of hate speech on social media and the urgent need for effective counter-measures have drawn significant investment from governments, companies, and researchers. A large number of methods have been developed for automated hate speech detection online. This aims to classify textual content into non-hate or hate speech, in which case the method may also identify the targeting characteristics (i.e., types of hate, such as race, and religion) in the hate speech. However, we notice significant difference between the performance of the two (i.e., non-hate v.s. hate). In this work, we argue for a focus on the latter problem for practical reasons. We show that it is a much more challenging task, as our analysis of the language in the typical datasets shows that hate speech lacks unique, discriminative features and therefore is found in the 'long tail' in a dataset that is difficult to discover. We then propose Deep Neural Network structures serving as feature extractors that are particularly effective for capturing the semantics of hate speech. Our methods are evaluated on the largest collection of hate speech datasets based on Twitter, and are shown to be able to outperform the best performing method by up to 5 percentage points in macro-average F1, or 8 percentage points in the more challenging case of identifying hateful content.

==> tables/tab_data_augmentation.tex <==
\begin{table}[thb]
    \centering
    \begin{tabular}{p{1.3cm}|p{0.8cm}|p{1.1cm}|p{1.1cm}|p{1.2cm}}
	%\begin{tabular}{c|c|c|c|c}
        \hline
        \textbf{Dataset} 		& \textbf{UoC(c\textsubscript{i})} 	& \textbf{Non-unique vocab.}	& \textbf{Shared Non-unique vocab.}	& \textbf{\% increase in training instances}\\
				\hline
	        
	        \multicolumn{5}{l}{\textbf{WZ-S.amt}}					\\\hline 
	        racism					& 112			& 724 		&\multirow{2}{*}{431}	&873\%\\ 
	        sexism					& 727			& 2,506 	&	&11\%\\ \hline
	        \multicolumn{5}{l}{\textbf{WZ-S.exp}}					\\\hline 
	        racism					& 106			& 518 		&\multirow{2}{*}{289}	&903\%\\ 
	        sexism					& 523			& 2,022 	&	&11\%\\ \hline
	        \multicolumn{5}{l}{\textbf{WZ-S.gb}}					\\\hline 
	        racism					& 101			& 515 		&\multirow{2}{*}{289}	&1026\%\\ 
	        sexism					& 627			& 2,235 	&	&10\%\\ \hline
	        \multicolumn{5}{l}{\textbf{WZ}}					\\\hline 
	        racism					& 408			& 2,621 	&\multirow{2}{*}{1,509}	&164\%\\ 
	        sexism					& 1,217			& 4,451 	&	&11\%\\ \hline
	        \multicolumn{5}{l}{\textbf{WZ.pj}}					\\\hline 
	        racism					& 427			& 2,826 	&\multirow{2}{*}{1,710}	&187\%\\ 
	        sexism					& 1,364			& 4,985 	&	&53\%\\

				\hline
			    \end{tabular}
		\caption{Statistics of the shared vocabulary (word stems) of the sexism and racism Tweets in each dataset and the number of new Tweets generated for each class in each dataset.}
		\label{tab_data_augmentation}
\end{table}

==> tables/tab_data_augmentation_example.tex <==
\begin{table*}[thb]
    \centering
    \begin{tabular}{p{7.3cm}|p{7.5cm}}
	%\begin{tabular}{c|c|c|c|c}
        \hline
        \textbf{Original Tweet (sexism)} 		&  \textbf{New Tweet (racism)}	\\\hline	      
	        \texttt{Those \textbf{bitchin, big-noting} \#MKR \textbf{babes} need to fall into an oven, cook better or shut the fuck up.}					&\texttt{Those \textbf{inscribes Mormon?} \#MKR \textbf{Kufiri} need to fall into an oven, cook better or shut the fuck up.}	\\
	        
	        \texttt{Drasco u are not a chef just a \textbf{wanka!} One day your misses will ask her self what the fuck am i doing with this dick?\#mkr}					&\texttt{Drasco u are not a chef just a \textbf{virtues}, One day your misses will ask her self what the fuck am i doing with this dick? \#mkr}	\\
	        
	        \texttt{Tonight's \#MKR confirms the casting people \textbf{trawl} the dark depths of the seriously delusional, the supremely misguided and plain rotten cooks.}	&\texttt{Tonight's \#MKR confirms the casting people \textbf{mafia} the dark depths of the seriously delusional, the supremely misguided and plain rotten cooks.}
				\\\hline 
		\textbf{Original Tweet (racism)} 		&  \textbf{New Tweet (sexism)}	\\\hline
			\texttt{of course you were born in \textbf{serbia...}you're as fucked as A \textbf{Serbian} Film \#MKR}	& \texttt{of course you were born in \textbf{COD} as fucked as A \textbf{righteous} Film \#MKR}\\
			
			\texttt{Man wtf is this damn \#Coon ass nigga \textbf{\#BillyBlanks} doing on that damn commercial? ? \textbf{\#CooneryAtItsFinest}
			}					& \texttt{Man wtf is this damn \#Coon ass nigga \textbf{\#FeminismAndCookies...} doing on that damn commercial? ? \textbf{metrosexual}}\\
			
			\texttt{@ummayman90 Exactly.  \textbf{\#Isam} is a cult of death centered around the idea of going to a heaven that is described to be a giant whore house.}					&  \texttt{@ummayman90 Exactly.  \textbf{Fleury} is a cult of death centered around the idea of going to a heaven that is described to be a giant whore house.} 	\\
				\hline
			    \end{tabular}
		\caption{Examples of generated Tweets from their original Tweets. The \textbf{bold} text highlights replaced words. }
		\label{tab_data_augmentation_example}
\end{table*}

==> tables/tab_errors.tex <==
\begin{table}[thb]
    \centering
%    \begin{tabular}{p{1.3cm}|c|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{3cm}}
    \begin{tabular}{c|c c c c c}
        \hline
        	& \textbf{Racism}	& \textbf{Sexism} 	& \textbf{Both}	&\textbf{Non-hate}	&\textbf{Hate}\\
				\hline
	WZ-S.amt	&25\%	&46\%	&3\%	&26\%	&N/A\\ 
				\hline 
	WZ-S.exp	&12\%	&52\%	&8\%	&28\%	&N/A	\\ 
				\hline 
	WZ-S.gb		&14\%	&50\%	&7\%	&29\%	&N/A	\\ 
				\hline 
  	WZ-LS		&23\%	&52\%	&1\%	&23\%	&N/A	\\ 
				\hline
	WZ-L	   	&22\%	&54\%	&N/A	&24\%	&N/A	\\ 				
				\hline
	DT			&N/A	&N/A	&N/A	&6\%	&94\%\\ 
				\hline
	RM			&N/A	&N/A	&N/A	&30\%	&70\%	\\ 
				\hline

    \end{tabular}
		\caption{Distribution of errors over all classes in each dataset.}
		\label{table_errors}
\end{table}




% 	WZ-L		&81.5	&81.0	&80.8	&80.7	&81.4	&80.5	&73.6	&74.2\\ 
%				\hline
%	WZ-S.amt	&90.2	&91.6	&89.4	&91.6	&90.1	&91.4	&86.2	&86.7\\ 
%				\hline 
%	WZ-S.exp	&90.4	&91.8	&90.1	&91.2	&90.4	&89.8	&89.1	&90.4\\ 
%				\hline 
%	WZ-S.gb		&91.1	&92.4	&90.0	&91.7	&90.9	&91.0	&86.2	&86.7\\ 
%				\hline 
%	WZ-LS   	&81.4	&82.1	&79.4	&81.3	&81.7	&81.3	&71.6	&72.5\\ 
%				\hline
%	DT			&93.9	&94.2	&92.3	&93.6	&93.1	&94.4	&86.6	&89.4\\ 
%				\hline
%	RM			&90.3	&91.8	&90.0	&90.6	&90.1	&90.1	&85.7	&88.7\\ 




==> tables/tab_f1_range.tex <==
\begin{table}[thb]
    \centering
    \begin{tabular}{p{0.7cm}|p{0.8cm}|p{0.8cm}|p{0.7cm}|p{1.2cm}|p{0.8cm}}
    %\begin{tabular}{c| c| c |c| c| c}
        \hline
        	& \textbf{Racism}	& \textbf{Sexism} 	& \textbf{Both}	&\textbf{Non-hate}	&\textbf{Hate}\\\hline
    
	WZ-S.amt	&.06$\sim$.4	&.66$\sim$.81	&0			&.88$\sim$.96	&-	\\ 
				\hline 
	WZ-S.exp	&.23$\sim$.56	&.57$\sim$.71	&0$\sim$.16	&.89$\sim$.95	&-	\\ 
				\hline 
	WZ-S.gb		&.16$\sim$.58	&.66$\sim$.79	&0$\sim$.17	&.88$\sim$.96	&-	\\ 
				\hline 
  	WZ.pj		&.55$\sim$.72	&.54$\sim$.69	&0$\sim$.12	&.78$\sim$.88	&-	\\ 
				\hline
	WZ	   		&.57$\sim$.74	&.53$\sim$.67	&-			&.78$\sim$.88   &-\\ 				
				\hline
	DT			&-		&-		&-		&.89$\sim$.98	&.24$\sim$.44	\\ 
				\hline
	RM			&-		&-		&-		&.91$\sim$.94	&.61$\sim$.67	\\ 
	
				\hline

    \end{tabular}
		\caption{Range of F1 obtained by different models.}
		\label{tab_f1_range}
\end{table}




% 	WZ-L		&81.5	&81.0	&80.8	&80.7	&81.4	&80.5	&73.6	&74.2\\ 
%				\hline
%	WZ-S.amt	&90.2	&91.6	&89.4	&91.6	&90.1	&91.4	&86.2	&86.7\\ 
%				\hline 
%	WZ-S.exp	&90.4	&91.8	&90.1	&91.2	&90.4	&89.8	&89.1	&90.4\\ 
%				\hline 
%	WZ-S.gb		&91.1	&92.4	&90.0	&91.7	&90.9	&91.0	&86.2	&86.7\\ 
%				\hline 
%	WZ-LS   	&81.4	&82.1	&79.4	&81.3	&81.7	&81.3	&71.6	&72.5\\ 
%				\hline
%	DT			&93.9	&94.2	&92.3	&93.6	&93.1	&94.4	&86.6	&89.4\\ 
%				\hline
%	RM			&90.3	&91.8	&90.0	&90.6	&90.1	&90.1	&85.7	&88.7\\ 




==> tables/tab_full_results_basecnn_datamix.tex <==
\begin{table*}[thb]
    \centering
    \begin{tabular}{p{1cm}|p{1.2cm}|p{0.2cm}p{0.2cm}p{0.2cm}|p{0.3cm}p{0.3cm}p{0.3cm}|p{0.3cm}p{0.3cm}p{0.3cm}|p{0.3cm}p{0.3cm}p{0.3cm}|p{.3cm}p{0.3cm}p{0.3cm}}
%    \begin{tabular}{c| c| c |c| c| c}
        \hline
        	\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Dataset and classes}}}& \multicolumn{3}{p{1.8cm}|}{\textbf{Base CNNs with e.none}} & \multicolumn{3}{p{1.8cm}|}{\textbf{Base CNNs with e.ggl}} & \multicolumn{3}{p{1.8cm}|}{\textbf{Base CNNs with e.twt}} & \multicolumn{3}{p{1.8cm}|}{\textbf{Base CNNs with e.glv}} & \multicolumn{3}{p{1.8cm}}{\textbf{Base CNNs with e.all}}\\\hline
        	
        	\multirow{5}{*}{WZ-S.amt}& 	& P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\\cline{2-17}
        			&racism 	&.25 &.14 &.17 &.25 &.13 &.16 &.22 &.13 &.15 &.3  &.16 &.2  &.23 &.13 &.15\\
        			&sexism 	&.82 &.71 &.76 &.84 &.76 &.7  &.85 &.74 &.79 &.85 &.75 &.8  &.85 &.74 &.8\\
        			&both 		&0   &0   &0   &0   &0   &0   &0   &0   &0   &0   &0   &0   &0   &0   &0\\
        			&non-hate 	&.93 &.96 &.94 &.94 &.97 &.95 &.95 &.97 &.95 &.93 &.97 &.95 &.93 &.97 &.95\\\hline
    		
    		\multirow{4}{*}{WZ-S.exp}
    		&racism 	&.3  &.27 &.28 &.39 &.32 &.35 &.44 &.23 &.3  &.34 &.23 &.27 &.41 &.22 &.29\\
    		&sexism 	&.7  &.58 &.64 &.73 &.63 &.67 &.69 &.62 &.66 &.71 &.65 &.68 &.69 &.63 &.66 \\
    		&both 	    &0   &0   &0   &.25 &.02 &.04 &.25 &.03 &.04 &.25 &.03 &.04 &.25 &.03 &.04\\
    		&non-hate 	&.93 &.96 &.95 &.94 &.97 &.95 &.94 &.96 &.95 &.94 &.96 &.95 &.94 &.96 &.95\\\hline
			
			\multirow{4}{*}{WZ-S.gb}
			&racism 	&.41 &.33 &.37 &.29 &.24 &.26 &.37 &.19 &.25 &.52 &.26 &.34 &.39 &.19 &.25\\
			&sexism 	&.76 &.67 &.71 &.8  &.73 &.76 &.81 &.71 &.76 &.8  &.7  &.75 &.81 &.71 &.75\\
			&both 	    &.15 &.07 &.09 &.25 &.03 &.05 &.25 &.03 &.05 &.25 &.03 &.05 &.25 &.03 &.05\\
			&non-hate 	&.94 &.96 &.95 &.94 &.96 &.95 &.94 &.97 &.96 &.94 &.97 &.96 &.94 &.97 &.96\\\hline
			
			\multirow{4}{*}{WZ.pj}
			&racism 	&.69 &.69 &.69 &.73 &.64 &.68 &.73 &.71 &.72 &.72 &.66 &.69 &.74 &.71 &.72\\
			&sexism		&.67 &.62 &.65 &.78 &.56 &.65 &.76 &.59 &.66 &.75 &.6  &.67 &.76 &.6  &.67\\
			&both 	    &.25 &.05 &.08 &0   &0   &0   &0   &0   &0   &0   &0   &0   &0   &0   &0\\
			&non-hate 	&.85 &.87 &.86 &.83 &.92 &.87 &.85 &.91 &.88 &.84 &.9  &.87 &.85 &.91 &.88\\\hline		
			
			\multirow{3}{*}{WZ}
			&racism 	&.63  &.67  &.65 &.67 &.65 &.66 &.71 &.64 &.67 &.69 &.64 &.67 &.71 &.64 &.67\\
			&sexism 	&.66  &.62  &.64 &.72 &.54 &.61 &.74 &.54 &.62 &.75 &.54 &.63 &.74 &.54 &.63\\			
			&non-hate 	&.84  &.85  &.88 &.83 &.89 &.86 &.83 &.9  &.86 &.83 &.9  &.86 &.83 &.9  &.86\\
				\hline

    \end{tabular}
		\caption{Full results obtained by the Base CNN models using the augmented training data. Results are shown for the part containing the original data only (i.e., synthetic data created by the augmentation process are excluded).}
		\label{tab_full_results_basecnn_datamix}
\end{table*}




% 	WZ-L		&81.5	&81.0	&80.8	&80.7	&81.4	&80.5	&73.6	&74.2\\ 
%				\hline
%	WZ-S.amt	&90.2	&91.6	&89.4	&91.6	&90.1	&91.4	&86.2	&86.7\\ 
%				\hline 
%	WZ-S.exp	&90.4	&91.8	&90.1	&91.2	&90.4	&89.8	&89.1	&90.4\\ 
%				\hline 
%	WZ-S.gb		&91.1	&92.4	&90.0	&91.7	&90.9	&91.0	&86.2	&86.7\\ 
%				\hline 
%	WZ-LS   	&81.4	&82.1	&79.4	&81.3	&81.7	&81.3	&71.6	&72.5\\ 
%				\hline
%	DT			&93.9	&94.2	&92.3	&93.6	&93.1	&94.4	&86.6	&89.4\\ 
%				\hline
%	RM			&90.3	&91.8	&90.0	&90.6	&90.1	&90.1	&85.7	&88.7\\ 




==> tables/tab_full_results_baselines-before-double-pooling.tex <==
\begin{table*}[thb]
    \centering
    	\caption{Full results obtained by all baseline models.}
    \begin{tabular}{p{1cm}|p{1.0cm}|p{0.2cm}p{0.2cm}p{0.2cm}|p{0.2cm}p{0.2cm}p{0.2cm}|p{0.2cm}p{0.2cm}p{0.2cm}|p{0.2cm}p{0.2cm}p{0.2cm}|p{.2cm}p{0.2cm}p{0.2cm}|p{.2cm}p{0.2cm}p{0.2cm}|p{0.2cm}p{0.2cm}p{0.2cm}}
%    \begin{tabular}{c| c| c |c| c| c}
        \hline
        	\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Dataset and classes}}}& \multicolumn{3}{c|}{\multirow{2}{*}{\textbf{SVM}}}	& 
        	\multicolumn{9}{c|}{\textbf{Gamback et al. \cite{Gamback2017}}}& 
        	\multicolumn{9}{c}{\textbf{Park et al. \cite{Park2017}}}\\\cline{6-23}
        	\multicolumn{2}{c|}{}&&&& \multicolumn{3}{c|}{e.w2v} & \multicolumn{3}{c|}{e.twt} & \multicolumn{3}{c|}{e.glv} & \multicolumn{3}{c|}{e.w2v} & \multicolumn{3}{c|}{e.twt} & \multicolumn{3}{c}{e.glv}\\\hline
        	
        	\multirow{4}{*}{WZ-S.amt}& 	& P &R &F & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\\cline{2-23}
        			&racism 	&.17 &.44 &.22 &.51 &.09 &.15 &.37 &.05 &.09 &.42 &.03 &.06 &.53 &.11 &.18 &.47 &.07 &.13 &.56 &.04 &.07\\
        			&sexism 	&.59 &.79 &.68 &.85 &.75 &.80 &.87 &.71 &.78 &.87 &.75 &.81 &.85 &.75 &.80 &.86 &.72 &.78 &.86 &.75 &.80\\        			
        			&non-hate 	&.95 &.82 &.88 &.93 &.97 &.95 &.92 &.98 &.95 &.93 &.98 &.95 &.93 &.97 &.95 &.93 &.98 &.95 &.93 &.98 &.95\\\hline
    		
    		\multirow{3}{*}{WZ-S.exp}
    		&racism 	&.21 &.51 &.26  &.61 &.41 &.49 &.58  &.31 &.40 &.53 &.18 &.26 &.59 &.38 &.46 &.56 &.26 &.35 &.57 &.21 &.31\\
    		&sexism 	&.46 &.76 &.58  &.74 &.58 &.65 &.75  &.60 &.67 &.74 &.61 &.67 &.74 &.58 &.65 &.75 &.59 &.66 &.73 &.61 &.67\\    		
    		&non-hate 	&.96 &.83 &.89  &.93 &.97 &.95 &.94  &.97 &.95 &.93 &.97 &.95 &.93 &.97 &.97 &.93 &.97 &.95 &.94 &.97 &.95\\\hline
			
			\multirow{3}{*}{WZ-S.gb}
			&racism 	&.28 &.70 &.38 &.53 &.30 &.38 &.53 &.22 &.31 &.61 &.21 &.31 &.48 &.30 &.37 &.57 &.22 &.31 &.64 &.22 &.33\\
			&sexism 	&.54 &.79 &.64 &.81 &.70 &.75 &.84 &.69 &.76 &.81 &.72 &.76 &.81 &.71 &.76 &.84 &.70 &.76 &.81 &.72 &.76\\			
			&non-hate 	&.96 &.85 &.90 &.94 &.97 &.96 &.94 &.98 &.96 &.94 &.97 &.96 &.94 &.97 &.96 &.94 &.98 &.96 &.94 &.97 &.96\\\hline
			
			\multirow{3}{*}{WZ.pj}
			&racism 	&.54 &.68 &.60 &.75 &.65 &.69 &.74 &.68 &.71 &.75 &.65 &.69 &.75 &.65 &.70 &.75 &.65 &.70 &.74 &.67 &.70\\
			&sexism 	&.51 &.66 &.58 &.77 &.60 &.67 &.77 &.59 &.67 &.78 &.57 &.66 &.77 &.60 &.68 &.78 &.57 &.66 &.77 &.57 &.68\\			
			&non-hate 	&.86 &.75 &.80 &.84 &.92 &.88 &.84 &.92 &.88 &.83 &.92 &.88 &.84 &.92 &.88 &.84 &.92 &.88 &.84 &.92 &.88\\\hline
			
			\multirow{3}{*}{WZ}
			&racism 	&.54 &.65 &.59 &.75 &.68 &.72 &.74 &.71 &.72  &.76 &.65 &.70 &.75 &.68 &.71 &.76 &.69 &.72&.76 &.67 &.71\\
			&sexism 	&.51 &.66 &.57 &.79 &.58 &.67 &.79 &.57 &.66  &.81 &.53 &.64 &.80 &.57 &.67 &.80 &.57 &.66&.81 &.53 &.64\\			
			&non-hate 	&.85 &.75 &.79 &.84 &.92 &.88 &.84 &.91 &.88  &.83 &.93 &.88 &.84 &.92 &.88 &.84 &.92 &.88 &.83 &.93 &.88\\\hline
			
			\multirow{2}{*}{DT}
			&hate 	    &.15 &.52 &.23 &.51 &.16 &.25 &.52 &.19 &.27 &.54 &.20 &.29 &.54 &.15 &.23 &.54 &.20 &.29 &.54 &.21 &.30\\					
			&non-hate 	&.97 &.81 &.88 &.95 &.99 &.97 &.95 &.99 &.97 &.95 &.99 &.97 &.95 &.99 &.97 &.95 &.99 &.97 &.95 &.99 &.97\\\hline
			
			\multirow{2}{*}{RM}
			&hate 	    &.45 &.81  &.58 &.74 &.62 &.67 &.75 &.57 &.65 &.76 &.59 &.66 &.75 &.62 &.68 &.76 &.56 &.64 &.74 &.59 &.66\\					
			&non-hate 	&.96 &.78 &.86  &.92 &.96 &.94 &.92 &.96 &.94 &.92 &.96 &.94 &.93 &.96 &.94 &.91 &.96 &.94 &.92 &.96 &.94\\
				\hline

    \end{tabular}
	
		\label{tab_full_results_baselines}
\end{table*}




% 	WZ-L		&81.5	&81.0	&80.8	&80.7	&81.4	&80.5	&73.6	&74.2\\ 
%				\hline
%	WZ-S.amt	&90.2	&91.6	&89.4	&91.6	&90.1	&91.4	&86.2	&86.7\\ 
%				\hline 
%	WZ-S.exp	&90.4	&91.8	&90.1	&91.2	&90.4	&89.8	&89.1	&90.4\\ 
%				\hline 
%	WZ-S.gb		&91.1	&92.4	&90.0	&91.7	&90.9	&91.0	&86.2	&86.7\\ 
%				\hline 
%	WZ-LS   	&81.4	&82.1	&79.4	&81.3	&81.7	&81.3	&71.6	&72.5\\ 
%				\hline
%	DT			&93.9	&94.2	&92.3	&93.6	&93.1	&94.4	&86.6	&89.4\\ 
%				\hline
%	RM			&90.3	&91.8	&90.0	&90.6	&90.1	&90.1	&85.7	&88.7\\ 




==> tables/tab_full_results_baselines-old.tex <==
\begin{table*}[thb]
    \centering
    \begin{tabular}{p{1cm}|p{1.2cm}|p{0.2cm}p{0.2cm}p{0.2cm}|p{0.2cm}p{0.2cm}p{0.2cm}|p{0.3cm}p{0.3cm}p{0.3cm}|p{0.3cm}p{0.3cm}p{0.3cm}|p{0.3cm}p{0.3cm}p{0.3cm}|p{.3cm}p{0.3cm}p{0.3cm}}
%    \begin{tabular}{c| c| c |c| c| c}
        \hline
        	\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Dataset and classes}}}& \multicolumn{3}{c|}{\multirow{2}{*}{\textbf{SVM}}}	& \multicolumn{3}{p{1.5cm}|}{\textbf{Base CNN with e.none}} & \multicolumn{3}{p{1.5cm}|}{\textbf{Base CNN with e.w2v}} & \multicolumn{3}{p{1.5cm}|}{\textbf{Base CNN with e.twt}} & \multicolumn{3}{p{1.5cm}|}{\textbf{Base CNN with e.glv}} & \multicolumn{3}{p{1.5cm}}{\textbf{Base CNN with e.all}}\\\hline
        	
        	\multirow{5}{*}{WZ-S.amt}& 	& P &R &F & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\\cline{2-20}
        			&racism 	&.16 &.39 &.22 &.35 &.12 &.17 &.38 &.08 &.13 &.33 &.03 &.06 &.45 &.04 &.07 &.37 &.04 &.07\\
        			&sexism 	&.58 &.78 &.66 &.79 &.7  &.74 &.85 &.75 &.80 &.86 &.71 &.78 &.87 &.74 &.80 &.87 &.71 &.78\\
        			&both 		&0 	 &0   &0   &0   &0   &0   &0   &0   &0   &0   &0   &0   &0   &0   &0   &0   &0   &0\\
        			&non-hate 	&.94 &.83 &.88 &.92 &.96 &.94 &.93 &.98 &.95 &.92 &.98 &.95 &.93 &.98 &.96 &.92 &.98 &.95\\\hline
    		
    		\multirow{4}{*}{WZ-S.exp}
    		&racism 	&.23 &.56 &.3  &.37 &.29 &.32 &.57 &.28 &.37 &.5  &.16 &.25 &.58 &.14 &.23 &.54 &.18 &.26\\
    		&sexism 	&.46 &.74 &.57 &.71 &.56 &.63 &.77 &.60 &.67 &.74 &.57 &.64 &.76 &.59 &.66 &.74 &.58 &.64\\
    		&both 	    &.29 &.23 &.16 &.17 &.04 &.07 &.25 &.02 &.04 &.25 &.02 &.04 &.25 &.02 &.04 &.25 &.02 &.04\\
    		&non-hate 	&.96 &.83 &.89 &.93 &.96 &.95 &.94 &.98 &.95 &.93 &.97 &.95 &.93 &.98 &.95 &.93 &.97 &.95\\\hline
			
			\multirow{4}{*}{WZ-S.gb}
			&racism 	&.26 &.67 &.35 &.51 &.36 &.42 &.53 &.24 &.33 &.37 &.10 &.16 &.56 &.13 &.22 &.43 &.13 &.2\\
			&sexism 	&.54 &.79 &.64 &.78 &.65 &.71 &.82 &.69 &.75 &.83 &.7  &.76 &.82 &.72 &.77 &.83 &.69 &.75\\
			&both 	    &.25 &.06 &.09 &.16 &.07 &.1  &.25 &.03 &.05 &.25 &.03 &.05 &.25 &.03 &.05 &.25 &.03 &.05\\
			&non-hate 	&.96 &.85 &.89 &.93 &.97 &.95 &.94 &.98 &.96 &.94 &.98 &.96 &.94 &.98 &.96 &.94 &.98 &.96\\\hline
			
			\multirow{4}{*}{WZ.pj}
			&racism 	&.49 &.63 &.55 &.71 &.65 &.68 &.74 &.62 &.68 &.75 &.63 &.69 &.75 &.61 &.67 &.75 &.64 &.69\\
			&sexism 	&.48 &.63 &.54 &.68 &.61 &.64 &.77 &.55 &.65 &.78 &.55 &.65 &.77 &.55 &.64 &.78 &.56 &.65\\
			&both 	    &.1  &.15 &.12 &.23 &.08 &.12 &0   &0   &0   &0   &0   &0   &0   &0   &0   &0   &0   &0\\
			&non-hate 	&.84 &.73 &.78 &.84 &.88 &.86 &.83 &.92 &.87 &.83 &.92 &.87 &.83 &.92 &.87 &.83 &.92 &.88\\\hline
			
			\multirow{3}{*}{WZ}
			&racism 	&.52 &.64 &.57 &.7  &.7  &.7  &.75 &.65 &.69 &.74 &.67 &.7  &.75 &.64 &.69 &.74 &.66 &.7\\
			&sexism 	&.47 &.62 &.53 &.7  &.6  &.64 &.79 &.53 &.63 &.79 &.54 &.64 &.81 &.53 &.64 &.79 &.55 &.65\\			
			&non-hate 	&.84 &.72 &.78 &.85 &.88 &.86 &.83 &.92 &.87 &.83 &.92 &.87 &.83 &.93 &.87 &.83 &.92 &.87\\\hline
			
			\multirow{2}{*}{DT}
			&hate 	    &.16 &.53 &.24 &.35 &.23 &.28 &.55 &.16 &.24 &.54 &.19 &.28 &.54 &.19 &.28 &.52 &.2  &.29\\					
			&non-hate 	&.97 &.82 &.89 &.95 &.97 &.96 &.95 &.99 &.98 &.95 &.99 &.97 &.95 &.99 &.97 &.95 &.99 &.97\\\hline
			
			\multirow{2}{*}{RM}
			&hate 	    &.48 &.8  &.59 &.66 &.57 &.61 &.76 &.59 &.66 &.73 &.53 &.61 &.76 &.58 &.66 &.73 &.54 &.62\\					
			&non-hate 	&.98 &.81 &.87 &.92 &.94 &.93 &.92 &.96 &.94 &.91 &.96 &.93 &.92 &.96 &.94 &.91 &.96 &.93\\
				\hline

    \end{tabular}
		\caption{Full results obtained by the SVM \cite{Davidson2017} and Base CNN models \cite{Gamback2017}) models.}
		\label{tab_full_results_baselines}
\end{table*}




% 	WZ-L		&81.5	&81.0	&80.8	&80.7	&81.4	&80.5	&73.6	&74.2\\ 
%				\hline
%	WZ-S.amt	&90.2	&91.6	&89.4	&91.6	&90.1	&91.4	&86.2	&86.7\\ 
%				\hline 
%	WZ-S.exp	&90.4	&91.8	&90.1	&91.2	&90.4	&89.8	&89.1	&90.4\\ 
%				\hline 
%	WZ-S.gb		&91.1	&92.4	&90.0	&91.7	&90.9	&91.0	&86.2	&86.7\\ 
%				\hline 
%	WZ-LS   	&81.4	&82.1	&79.4	&81.3	&81.7	&81.3	&71.6	&72.5\\ 
%				\hline
%	DT			&93.9	&94.2	&92.3	&93.6	&93.1	&94.4	&86.6	&89.4\\ 
%				\hline
%	RM			&90.3	&91.8	&90.0	&90.6	&90.1	&90.1	&85.7	&88.7\\ 




==> tables/tab_full_results_baselines-withe.none.tex <==
\begin{table}[thb]
    \centering
    \begin{tabular}{p{1cm}|p{1.0cm}|p{0.2cm}p{0.2cm}p{0.2cm}|p{0.3cm}p{0.3cm}p{0.3cm}|p{0.3cm}p{0.3cm}p{0.3cm}|p{0.3cm}p{0.3cm}p{0.3cm}|p{.3cm}p{0.3cm}p{0.3cm}|p{.3cm}p{0.3cm}p{0.3cm}|p{.3cm}p{0.3cm}p{0.3cm}}
%    \begin{tabular}{c| c| c |c| c| c}
        \hline
        	\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Dataset and classes}}}& \multicolumn{3}{c|}{\multirow{2}{*}{\textbf{SVM}}}	& 
        	\multicolumn{9}{c|}{\textbf{Gamback et al. \cite{Gamback2017}}}& 
        	\multicolumn{9}{c}{\textbf{Park et al. \cite{Park2017}}}\\\cline{6-23}
        	\multicolumn{2}{c|}{}&&&& \multicolumn{3}{p{1.5cm}|}{e.w2v} & \multicolumn{3}{p{1.5cm}|}{e.twt} & \multicolumn{3}{p{1.5cm}|}{e.glv} & \multicolumn{3}{p{1.5cm}|}{e.w2v} & \multicolumn{3}{p{1.5cm}|}{e.twt} & \multicolumn{3}{p{1.5cm}}{e.glv}\\\hline
        	
        	\multirow{4}{*}{WZ-S.amt}& 	& P &R &F & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\\cline{2-23}
        			&racism 	&.17 &.44 &.22 &.22 &.08 &.12 &.51 &.09 &.15 &.37 &.05 &.09 &.42 &.03 &.06 &.31 &.14 &.19 &.53 &.11 &.18 &.47 &.08 &.13 &.56 &.04 &.07\\
        			&sexism 	&.59 &.79 &.68 &.80 &.71 &.75 &.85 &.75 &.80 &.87 &.71 &.78 &.87 &.75 &.81 &.79 &.71 &.75 &.85 &.75 &.80 &.86 &.72 &.78 &.86 &.75 &.80\\        			
        			&non-hate 	&.95 &.82 &.88 &.93 &.96 &.94 &.93 &.97 &.95 &.92 &.98 &.95 &.93 &.98 &.95 &.93 &.96 &.94 &.93 &.97 &.95 &.93 &.98 &.95 &.93 &.98 &.95\\\hline
    		
    		\multirow{3}{*}{WZ-S.exp}
    		&racism 	&.21 &.51 &.26  &.48 &.31 &.38 &.61 &.41 &.49 &.58  &.31 &.40 &.53 &.18 &.26 &.44 &.34 &.38 &.59 &.38 &.46 &.56 &.26 &.35 &.57 &.21 &.31\\
    		&sexism 	&.46 &.76 &.58  &.71 &.57 &.63 &.74 &.58 &.65 &.75  &.60 &.67 &.74 &.61 &.67 &.72 &.56 &.63 &.74 &.58 &.65 &.75 &.59 &.66 &.73 &.61 &.67\\    		
    		&non-hate 	&.96 &.83 &.89  &.93 &.97 &.95 &.93 &.97 &.95 &.94  &.97 &.95 &.93 &.97 &.95 &.93 &.97 &.95 &.93 &.97 &.97 &.93 &.97 &.95 &.94 &.97 &.95\\\hline
			
			\multirow{3}{*}{WZ-S.gb}
			&racism 	&.28 &.70 &.38 &.49 &.32 &.39 &.53 &.30 &.38 &.53 &.22 &.31 &.61 &.21 &.31 &.53 &.34 &.41 &.48 &.30 &.37 &.57 &.22 &.31 &.64 &.22 &.33\\
			&sexism 	&.54 &.79 &.64 &.78 &.65 &.70 &.81 &.70 &.75 &.84 &.69 &.76 &.81 &.72 &.76 &.78 &.64 &.70 &.81 &.71 &.76 &.84 &.70 &.76 &.81 &.72 &.76\\			
			&non-hate 	&.96 &.85 &.90 &.93 &.97 &.95 &.94 &.97 &.96 &.94 &.98 &.96 &.94 &.97 &.96 &.93 &.97 &.95 &.94 &.97 &.96 &.94 &.98 &.96 &.94 &.97 &.96\\\hline
			
			\multirow{3}{*}{WZ.pj}
			&racism 	&.54 &.68 &.60 &.70 &.65 &.68 &.75 &.65 &.69 &.74 &.68 &.71 &.75 &.65 &.69 &.71 &.65 &.68 &.75 &.65 &.70 &.75 &.65 &.70 &.74 &.67 &.70\\
			&sexism 	&.51 &.66 &.58 &.68 &.62 &.65 &.77 &.60 &.67 &.77 &.59 &.67 &.78 &.57 &.66 &.68 &.60 &.64 &.77 &.60 &.68 &.78 &.57 &.66 &.77 &.57 &.68\\			
			&non-hate 	&.86 &.75 &.80 &.84 &.88 &.86 &.84 &.92 &.88 &.84 &.92 &.88 &.83 &.92 &.88 &.84 &.88 &.86 &.84 &.92 &.88 &.84 &.92 &.88 &.84 &.92 &.88\\\hline
			
			\multirow{3}{*}{WZ}
			&racism 	&.54 &.65 &.59 &.70  &.66  &.68  &.75 &.68 &.72 &.74 &.71 &.72  &.76 &.65 &.70 &.71 &.66 &.68 &.75 &.68 &.71 &.76 &.69 &.72&.76 &.67 &.71\\
			&sexism 	&.51 &.66 &.57 &.68  &.60  &.64  &.79 &.58 &.67 &.79 &.57 &.66  &.81 &.53 &.64 &.68 &.61 &.65 &.80 &.57 &.67 &.80 &.57 &.66&.81 &.53 &.64\\			
			&non-hate 	&.85 &.75 &.79 &.84  &.87  &.86  &.84 &.92 &.88 &.84 &.91 &.88  &.83 &.93 &.88 &.84 &.88 &.86 &.84 &.92 &.88 &.84 &.92 &.88 &.83 &.93 &.88\\\hline
			
			\multirow{2}{*}{DT}
			&hate 	    &.15 &.52 &.23 &.36 &.24 &.29 &.51 &.16 &.25 &.52 &.19 &.27 &.54 &.20 &.29 &.36 &.24  &.29 &.54 &.15 &.23 &.54 &.20 &.29 &.54 &.21 &.30\\					
			&non-hate 	&.97 &.81 &.88 &.95 &.97 &.96 &.95 &.99 &.97 &.95 &.99 &.97 &.95 &.99 &.97 &.95 &.97  &.96 &.95 &.99 &.97 &.95 &.99 &.97 &.95 &.99 &.97\\\hline
			
			\multirow{2}{*}{RM}
			&hate 	    &.45 &.81  &.58 &.65 &.57 &.61 &.74 &.62 &.67 &.75 &.57 &.65 &.76 &.59 &.66 &.66 &.56 &.61 &.75 &.62 &.68 &.76 &.56 &.64 &.74 &.59 &.66\\					
			&non-hate 	&.96 &.78 &.86  &.92 &.94 &.93 &.92 &.96 &.94 &.92 &.96 &.94 &.92 &.96 &.94 &.91 &.94 &.93 &.93 &.96 &.94 &.91 &.96 &.94 &.92 &.96 &.94\\
				\hline

    \end{tabular}
		\caption{Full results obtained by all baseline models.}
		\label{tab_full_results_baselines}
\end{table}




% 	WZ-L		&81.5	&81.0	&80.8	&80.7	&81.4	&80.5	&73.6	&74.2\\ 
%				\hline
%	WZ-S.amt	&90.2	&91.6	&89.4	&91.6	&90.1	&91.4	&86.2	&86.7\\ 
%				\hline 
%	WZ-S.exp	&90.4	&91.8	&90.1	&91.2	&90.4	&89.8	&89.1	&90.4\\ 
%				\hline 
%	WZ-S.gb		&91.1	&92.4	&90.0	&91.7	&90.9	&91.0	&86.2	&86.7\\ 
%				\hline 
%	WZ-LS   	&81.4	&82.1	&79.4	&81.3	&81.7	&81.3	&71.6	&72.5\\ 
%				\hline
%	DT			&93.9	&94.2	&92.3	&93.6	&93.1	&94.4	&86.6	&89.4\\ 
%				\hline
%	RM			&90.3	&91.8	&90.0	&90.6	&90.1	&90.1	&85.7	&88.7\\ 




==> tables/tab_full_results_cnn_gru.tex <==
\begin{table*}[thb]
    \centering
    \begin{tabular}{p{1cm}|p{1.2cm}|p{0.2cm}p{0.2cm}p{0.2cm}|p{0.3cm}p{0.3cm}p{0.3cm}|p{0.3cm}p{0.3cm}p{0.3cm}|p{0.3cm}p{0.3cm}p{0.3cm}|p{.3cm}p{0.3cm}p{0.3cm}}
%    \begin{tabular}{c| c| c |c| c| c}
        \hline
        	\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Dataset and classes}}}& \multicolumn{3}{p{1.8cm}|}{\textbf{Base CNN+GRU with e.none}} & \multicolumn{3}{p{1.8cm}|}{\textbf{Base CNN+GRUs with e.w2v}} & \multicolumn{3}{p{1.8cm}|}{\textbf{Base CNN+GRU with e.twt}} & \multicolumn{3}{p{1.8cm}|}{\textbf{Base CNN+GRU with e.glv}} & \multicolumn{3}{p{1.8cm}}{\textbf{Base CNN+GRU with e.all}}\\\hline
        	
        	\multirow{5}{*}{WZ-S.amt}& 	& P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\\cline{2-17}
        			&racism 	&.28 &.21 &.24 &.36 &.12 &.18 &.5  &.1  &.17 &.34 &.08 &.13 &.4  &.11 &.17\\
        			&sexism 	&.77 &.75 &.76 &.86 &.75 &.8  &.86 &.74 &.8  &.85 &.78 &.81 &.86 &.74 &.8\\
        			&both 		&0   &0   &0   &0   &0   &0   &0   &0   &0   &0   &0   &0   &0   &0   &0\\
        			&non-hate 	&.93 &.95 &.94 &.93 &.97 &.95 &.93 &.98 &.95 &.94 &.97 &.96 &.93 &.98 &.95\\\hline
    		
    		\multirow{4}{*}{WZ-S.exp}
    		&racism 	&.48 &.37 &.42 &.53 &.44 &.48 &.47 &.23 &.31 &.66 &.27 &.38 &.46 &.21 &.29\\
    		&sexism 	&.7  &.55 &.62 &.72 &.65 &.68 &.75 &.61 &.67 &.71 &.66 &.68 &.74 &.63 &.68 \\
    		&both 	    &.13 &.04 &.06 &0   &0   &0   &.25 &.06 &.1  &0   &0   &0   &.25 &.04 &.07\\
    		&non-hate 	&.93 &.96 &.95 &.94 &.96 &.95 &.94 &.97 &.95 &.95 &.95 &.95 &.94 &.97 &.95\\\hline
			
			\multirow{4}{*}{WZ-S.gb}
			&racism 	&.53 &.42 &.47 &.63 &.45 &.53 &.56 &.32 &.48 &.58 &.23 &.33 &.52 &.32 &.4\\
			&sexism 	&.73 &.7  &.71 &.78 &.76 &.77 &.81 &.75 &.78 &.79 &.75 &.77 &.8  &.74 &.77\\
			&both 	    &.13 &.03 &.05 &0   &0   &0   &.25 &.03 &.05 &0   &0   &0   &.25 &.03 &.05\\
			&non-hate 	&.94 &.96 &.95 &.96 &.97 &.96 &.95 &.97 &.96 &.95 &.97 &.96 &.95 &.97 &.96\\\hline
			
			\multirow{4}{*}{WZ.pj}
			&racism 	&.69 &.69 &.69 &.73 &.64 &.68 &.73 &.71 &.72 &.72 &.66 &.69 &.74 &.71 &.72\\
			&sexism		&.67 &.62 &.65 &.78 &.56 &.65 &.76 &.59 &.66 &.75 &.6  &.67 &.76 &.6  &.67\\
			&both 	    &.25 &.05 &.08 &0   &0   &0   &0   &0   &0   &0   &0   &0   &0   &0   &0\\
			&non-hate 	&.85 &.87 &.86 &.83 &.92 &.87 &.85 &.91 &.88 &.84 &.9  &.87 &.85 &.91 &.88\\\hline		
			
			\multirow{3}{*}{WZ}
			&racism 	&.7   &.7   &.7  &.73 &.63 &.68 &.72 &.71 &.71 &.72 &.72 &.72 &.73 &.73 &.72\\
			&sexism 	&.7   &.61  &.65 &.85 &.48 &.61 &.82 &.49 &.61 &.79 &.56 &.66 &.82 &.5  &.62\\			
			&non-hate 	&.85  &.88  &.86 &.82 &.94 &.87 &.83 &.92 &.87 &.84 &.91 &.87 &.83 &.92 &.87\\\hline
			
			\multirow{2}{*}{DT}
			&hate 	    &.34 &.28 &.3  &.43 &.22 &.29 &.46 &.29 &.36 &.54 &.24 &.32 &.45 &.31 &.36\\					
			&non-hate 	&.96 &.97 &.96 &.95 &.98 &.97 &.96 &.98 &.97 &.96 &.99 &.97 &.96 &.98 &.97\\\hline
			
			\multirow{2}{*}{RM}
			&hate 	    &.65 &.59 &.61 &.74 &.6  &.66  &.75 &.6  &.67 &.77 &.59 &.66 &.74 &.59 &.66\\					
			&non-hate 	&.92 &.93 &.93 &.92 &.96 &.94  &.92 &.96 &.94 &.92 &.96 &.94 &.92 &.96 &.94\\
				\hline

    \end{tabular}
		\caption{Full results obtained by the Base+GRU models.}
		\label{tab_full_results_cnn_skipped}
\end{table*}




% 	WZ-L		&81.5	&81.0	&80.8	&80.7	&81.4	&80.5	&73.6	&74.2\\ 
%				\hline
%	WZ-S.amt	&90.2	&91.6	&89.4	&91.6	&90.1	&91.4	&86.2	&86.7\\ 
%				\hline 
%	WZ-S.exp	&90.4	&91.8	&90.1	&91.2	&90.4	&89.8	&89.1	&90.4\\ 
%				\hline 
%	WZ-S.gb		&91.1	&92.4	&90.0	&91.7	&90.9	&91.0	&86.2	&86.7\\ 
%				\hline 
%	WZ-LS   	&81.4	&82.1	&79.4	&81.3	&81.7	&81.3	&71.6	&72.5\\ 
%				\hline
%	DT			&93.9	&94.2	&92.3	&93.6	&93.1	&94.4	&86.6	&89.4\\ 
%				\hline
%	RM			&90.3	&91.8	&90.0	&90.6	&90.1	&90.1	&85.7	&88.7\\ 




==> tables/tab_full_results_cnn_skipped.tex <==
\begin{table*}[thb]
    \centering
    \begin{tabular}{p{1cm}|p{1.2cm}|p{0.2cm}p{0.2cm}p{0.2cm}|p{0.3cm}p{0.3cm}p{0.3cm}|p{0.3cm}p{0.3cm}p{0.3cm}|p{0.3cm}p{0.3cm}p{0.3cm}|p{.3cm}p{0.3cm}p{0.3cm}}
%    \begin{tabular}{c| c| c |c| c| c}
        \hline
        	\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Dataset and classes}}}& \multicolumn{3}{p{1.8cm}|}{\textbf{Base CNN+sCNN with e.none}} & \multicolumn{3}{p{1.8cm}|}{\textbf{Base CNN+sCNN with e.w2v}} & \multicolumn{3}{p{1.8cm}|}{\textbf{Base CNN+sCNN with e.twt}} & \multicolumn{3}{p{1.8cm}|}{\textbf{Base CNN+sCNN with e.glv}} & \multicolumn{3}{p{1.8cm}}{\textbf{Base CNN+sCNN with e.all}}\\\hline
        	
        	\multirow{5}{*}{WZ-S.amt}& 	& P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\\cline{2-17}
        			&racism 	&.34 &.22 &.26 &.44 &.39 &.40 &.46 &.26 &.33 &.34 &.14 &.2  &.46 &.26 &.33\\
        			&sexism 	&.77 &.75 &.76 &.79 &.83 &.81 &.8  &.8  &.8  &.81 &.8  &.81 &.79 &.8  &.79\\
        			&both 		&0   &0   &0   &0   &0   &0   &0   &0   &0   &0   &0   &0   &0   &0   &0\\
        			&non-hate 	&.93 &.95 &.94 &.95 &.95 &.95 &.95 &.96 &.95 &.94 &.96 &.95 &.94 &.95 &.95\\\hline
    		
    		\multirow{4}{*}{WZ-S.exp}
    		&racism 	&.46 &.45 &.45 &.48 &.67 &.56 &.46 &.58 &.51 &.48 &.51 &.49 &.46 &.58 &.51\\
    		&sexism 	&.71 &.55 &.62 &.68 &.75 &.71 &.67 &.74 &.7  &.7  &.73 &.72 &.67 &.74 &.7 \\
    		&both 	    &.15 &.06 &.09 &.25 &.06 &.1  &.25 &.06 &.1  &.25 &.02 &.04 &.25 &.06 &.1\\
    		&non-hate 	&.93 &.96 &.95 &.96 &.94 &.95 &.96 &.94 &.95 &.95 &.95 &.95 &.96 &.94 &.95\\\hline
			
			\multirow{4}{*}{WZ-S.gb}
			&racism 	&.48 &.48 &.48 &.49 &.7  &.58 &.49 &.56 &.52 &.48 &.47 &.47 &.5  &.57 &.53\\
			&sexism 	&.76 &.68 &.71 &.75 &.8  &.77 &.77 &.78 &.77 &.79 &.78 &.79 &.77 &.78 &.78\\
			&both 	    &.37 &.13 &.17 &.15 &.08 &.11 &.25 &.06 &.09 &.17 &.06 &.08 &.25 &.03 &.05\\
			&non-hate 	&.94 &.96 &.95 &.96 &.95 &.96 &.96 &.96 &.96 &.96 &.96 &.96 &.96 &.96 &.96\\\hline
			
			\multirow{4}{*}{WZ.pj}
			&racism 	&.7  &.69 &.69 &.64 &.8  &.71 &.64 &.85 &.73 &.69 &.75 &.72 &.64 &.85 &.73\\
			&sexism		&.66 &.64 &.65 &.65 &.69 &.67 &.66 &.69 &.68 &.71 &.66 &.69 &.67 &.69 &.68\\
			&both 	    &.11 &.07 &.09 &.25 &.05 &.08 &.25 &.03 &.05 &0   &0   &0   &.19 &.08 &.11\\
			&non-hate 	&.85 &.86 &.86 &.88 &.83 &.85 &.88 &.83 &.85 &.87 &.87 &.87 &.88 &.93 &.86\\\hline		
			
			\multirow{3}{*}{WZ}
			&racism 	&.69  &.72  &.7  &.65 &.81 &.72 &.64 &.87 &.74 &.69 &.78 &.74 &.64 &.87 &.74\\
			&sexism 	&.67  &.63  &.65 &.70 &.63 &.66 &.71 &.63 &.67 &.74 &.62 &.67 &.71 &.63 &.67\\			
			&non-hate 	&.85  &.86  &.86 &.86 &.85 &.86 &.87 &.85 &.86 &.86 &.88 &.87 &.87 &.85 &.86\\\hline
			
			\multirow{2}{*}{DT}
			&hate 	    &.37 &.24 &.29 &.48 &.24 &.32 &.49 &.35 &.41 &.49 &.4  &.44 &.46 &.4  &.43\\					
			&non-hate 	&.95 &.97 &.96 &.95 &.98 &.97 &.96 &.98 &.97 &.96 &.97 &.97 &.96 &.97 &.97\\\hline
			
			\multirow{2}{*}{RM}
			&hate 	    &.66 &.61 &.63 &.64 &.78 &.7  &.64 &.76 &.69 &.7  &.71 &.7  &.64 &.76 &.69\\					
			&non-hate 	&.92 &.94 &.93 &.95 &.91 &.93 &.95 &.91 &.93 &.94 &.94 &.94 &.95 &.91 &.93\\
				\hline

    \end{tabular}
		\caption{Full results obtained by the Base+sCNN models.}
		\label{tab_full_results_cnn_skipped}
\end{table*}




% 	WZ-L		&81.5	&81.0	&80.8	&80.7	&81.4	&80.5	&73.6	&74.2\\ 
%				\hline
%	WZ-S.amt	&90.2	&91.6	&89.4	&91.6	&90.1	&91.4	&86.2	&86.7\\ 
%				\hline 
%	WZ-S.exp	&90.4	&91.8	&90.1	&91.2	&90.4	&89.8	&89.1	&90.4\\ 
%				\hline 
%	WZ-S.gb		&91.1	&92.4	&90.0	&91.7	&90.9	&91.0	&86.2	&86.7\\ 
%				\hline 
%	WZ-LS   	&81.4	&82.1	&79.4	&81.3	&81.7	&81.3	&71.6	&72.5\\ 
%				\hline
%	DT			&93.9	&94.2	&92.3	&93.6	&93.1	&94.4	&86.6	&89.4\\ 
%				\hline
%	RM			&90.3	&91.8	&90.0	&90.6	&90.1	&90.1	&85.7	&88.7\\ 




==> tables/tab_full_results_datamix.tex <==
\begin{table*}[thb]
    \centering
    \begin{tabular}{p{1cm}|p{1.2cm}|p{0.2cm}p{0.2cm}p{0.2cm}|p{0.2cm}p{0.2cm}p{0.2cm}|p{0.3cm}p{0.3cm}p{0.3cm}|p{0.3cm}p{0.3cm}p{0.3cm}|p{0.3cm}p{0.3cm}p{0.3cm}|p{.3cm}p{0.3cm}p{0.3cm}}
%    \begin{tabular}{c| c| c |c| c| c}
        \hline
        	\multicolumn{2}{c|}{Dataset and classes}& \multicolumn{3}{c|}{\textbf{SVM}}	& \multicolumn{3}{p{1.5cm}|}{\textbf{Base CNNs with e.none}} & \multicolumn{3}{p{1.5cm}|}{\textbf{Base CNNs with e.ggl}} & \multicolumn{3}{p{1.5cm}|}{\textbf{Base CNNs with e.twt}} & \multicolumn{3}{p{1.5cm}|}{\textbf{Base CNNs with e.glv}} & \multicolumn{3}{p{1.5cm}}{\textbf{Base CNNs with e.all}}\\\hline
        	
        	\multirow{4}{*}{WZ-S.amt}& 	& P &R &F & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\\cline{2-20}
        			&racism 	&.81 &.81 &.81 & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\
        			&sexism 	&.81 &.81 &.81 & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\
        			&both 	&.81 &.81 &.81 & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\
        			&non-hate 	&.81 &.81 &.81 & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\\hline
    		
    		\multirow{4}{*}{WZ-S.exp}& 	& P &R &F & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\\cline{2-20}
    		&racism 	&.81 &.81 &.81 & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\
    		&sexism 	&.81 &.81 &.81 & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\
    		&both 	&.81 &.81 &.81 & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\
    		&non-hate 	&.81 &.81 &.81 & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\\hline
			
			\multirow{4}{*}{WZ-S.gb}& 	& P &R &F & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\\cline{2-20}
			&racism 	&.81 &.81 &.81 & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\
			&sexism 	&.81 &.81 &.81 & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\
			&both 	&.81 &.81 &.81 & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\
			&non-hate 	&.81 &.81 &.81 & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\\hline
			
			\multirow{4}{*}{WZ.pj}& 	& P &R &F & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\\cline{2-20}
			&racism 	&.81 &.81 &.81 & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\
			&sexism 	&.81 &.81 &.81 & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\
			&both 	&.81 &.81 &.81 & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\
			&non-hate 	&.81 &.81 &.81 & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\\hline
			
			\multirow{3}{*}{WZ}& 	& P &R &F & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\\cline{2-20}
			&racism 	&.81 &.81 &.81 & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\
			&sexism 	&.81 &.81 &.81 & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\			
			&non-hate 	&.81 &.81 &.81 & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\\hline
			
			\multirow{2}{*}{DT}& 	& P &R &F & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\\cline{2-20}
			&hate 	&.81 &.81 &.81 & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\					
			&non-hate 	&.81 &.81 &.81 & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\\hline
			
			\multirow{2}{*}{RM}& 	& P &R &F & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\\cline{2-20}
			&hate 	&.81 &.81 &.81 & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\					
			&non-hate 	&.81 &.81 &.81 & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\
				\hline

    \end{tabular}
		\caption{Full results obtained by the SVM \cite{Davidson2017} and Base CNNs \cite{Gamback2017}) models.}
		\label{tab_full_results_baselines}
\end{table*}




% 	WZ-L		&81.5	&81.0	&80.8	&80.7	&81.4	&80.5	&73.6	&74.2\\ 
%				\hline
%	WZ-S.amt	&90.2	&91.6	&89.4	&91.6	&90.1	&91.4	&86.2	&86.7\\ 
%				\hline 
%	WZ-S.exp	&90.4	&91.8	&90.1	&91.2	&90.4	&89.8	&89.1	&90.4\\ 
%				\hline 
%	WZ-S.gb		&91.1	&92.4	&90.0	&91.7	&90.9	&91.0	&86.2	&86.7\\ 
%				\hline 
%	WZ-LS   	&81.4	&82.1	&79.4	&81.3	&81.7	&81.3	&71.6	&72.5\\ 
%				\hline
%	DT			&93.9	&94.2	&92.3	&93.6	&93.1	&94.4	&86.6	&89.4\\ 
%				\hline
%	RM			&90.3	&91.8	&90.0	&90.6	&90.1	&90.1	&85.7	&88.7\\ 




==> tables/tab_full_results_dnnplus-withe.none.tex <==
\begin{table}[thb]
    \centering
    \begin{tabular}{p{1cm}|p{1.0cm}|p{0.2cm}p{0.2cm}p{0.2cm}|p{0.3cm}p{0.3cm}p{0.3cm}|p{0.3cm}p{0.3cm}p{0.3cm}|p{0.3cm}p{0.3cm}p{0.3cm}|p{.3cm}p{0.3cm}p{0.3cm}|p{.3cm}p{0.3cm}p{0.3cm}|p{.3cm}p{0.3cm}p{0.3cm}|p{.3cm}p{0.3cm}p{0.3cm}}
%    \begin{tabular}{c| c| c |c| c| c}
        \hline
        	\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Dataset and classes}}}&  
        	\multicolumn{12}{c|}{\textbf{CNN+sCNN}}& 
        	\multicolumn{12}{c}{\textbf{CNN+GRU}}\\\cline{3-26}
        	\multicolumn{2}{c|}{}&\multicolumn{3}{p{1.5cm}|}{e.none} & \multicolumn{3}{p{1.5cm}|}{e.w2v} & \multicolumn{3}{p{1.5cm}|}{e.twt} & \multicolumn{3}{p{1.5cm}|}{e.glv} & \multicolumn{3}{p{1.5cm}|}{e.none} & \multicolumn{3}{p{1.5cm}|}{e.w2v} & \multicolumn{3}{p{1.5cm}|}{e.twt} & \multicolumn{3}{p{1.5cm}}{e.glv}\\\hline
        	
        	\multirow{4}{*}{WZ-S.amt}& 	& P &R &F & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\\cline{2-26}
        			&racism 	&.37 &.27 &.31 &.45 &.22 &.29 &.43 &.26 &.32 &.36 &.21 &.26 &.34 &.26 &.29 &.44 &.14 &.21 &.44 &.15 &.22 &.48 &.18 &.26\\
        			&sexism 	&.76 &.75 &.76 &.84 &.78 &.81 &.80 &.79 &.79 &.81 &.81 &.81 &.76 &.76 &.76 &.84 &.75 &.80 &.86 &.74 &.79 &.83 &.77 &.80\\        			
        			&non-hate 	&.94 &.94 &.94 &.94 &.97 &.95 &.94 &.96 &.95 &.95 &.96 &.95 &.94 &.94 &.94 &.93 &.97 &.95 &.93 &.97 &.95 &.94 &.97 &.95\\\hline
    		
    		\multirow{3}{*}{WZ-S.exp}
    		&racism 	&.44 &.44 &.44 &.60 &.57 &.58 &.59  &.67 &.63 &.52 &.64 &.57 &.50 &.45 &.48 &.52 &.48 &.50 &.58 &.26 &.36 &.50 &.26 &.34\\
    		&sexism 	&.72 &.57 &.64 &.72 &.65 &.68 &.68  &.76 &.72 &.67 &.74 &.70 &.71 &.56 &.63 &.67 &.64 &.65 &.75 &.60 &.67 &.74 &.61 &.67\\    		
    		&non-hate 	&.93 &.97 &.95 &.93 &.95 &.96 &.96  &.95 &.95 &.96 &.95 &.95 &.93 &.96 &.95 &.94 &.96 &.95 &.93 &.97 &.95 &.94 &.97 &.95\\\hline
			
			\multirow{3}{*}{WZ-S.gb}
			&racism 	&.53 &.61 &.57 &.55 &.53 &.54 &.53 &.63 &.58 &.50 &.52 &.51 &.52 &.51 &.51 &.54 &.47 &.50 &.62 &.38 &.47 &.66 &.34 &.45\\
			&sexism 	&.78 &.65 &.70 &.82 &.73 &.77 &.78 &.79 &.79 &.78 &.80 &.79 &.74 &.73 &.73 &.79 &.76 &.77 &.82 &.74 &.78 &.81 &.75 &.78\\			
			&non-hate 	&.94 &.96 &.95 &.94 &.97 &.96 &.96 &.96 &.96 &.96 &.96 &.96 &.95 &.96 &.95 &.95 &.96 &.96 &.95 &.97 &.96 &.95 &.97 &.96\\\hline
			
			\multirow{3}{*}{WZ.pj}
			&racism 	&.69 &.68 &.69 &.72 &.73 &.73 &.64 &.86 &.74 &.69 &.80 &.74 &.69 &.67 &.68 &.73 &.67 &.70 &.73 &.72 &.72 &.72 &.76 &.74\\
			&sexism 	&.67 &.63 &.65 &.75 &.64 &.69 &.69 &.71 &.70 &.70 &.67 &.68 &.66 &.63 &.64 &.76 &.61 &.68 &.75 &.62 &.68 &.75 &.62 &.68\\			
			&non-hate 	&.85 &.86 &.86 &.86 &.90 &.88 &.89 &.84 &.86 &.87 &.87 &.87 &.85 &.87 &.86 &.85 &.91 &.88 &.85 &.90 &.88 &.86 &.90 &.88\\\hline
			
			\multirow{3}{*}{WZ}
			&racism 	&.69  &.69  &.69  &.73 &.74 &.74 &.64 &.87 &.74  &.69 &.84 &.76 &.68 &.67 &.68 &.75 &.70 &.73 &.74 &.74 &.74&.74 &.72 &.73\\
			&sexism 	&.68  &.61  &.65  &.79 &.59 &.68 &.73 &.63 &.68  &.73 &.63 &.68 &.65 &.64 &.65 &.76 &.62 &.68 &.76 &.59 &.67&.78 &.57 &.66\\			
			&non-hate 	&.84  &.87  &.86  &.85 &.91 &.88 &.87 &.86 &.87  &.87 &.87 &.87 &.84 &.85 &.85 &.85 &.91 &.88 &.85 &.90 &.88 &.84 &.91 &.88\\\hline
			
			\multirow{2}{*}{DT}
			&hate 	    &.37 &.27 &.32 &.51 &.21 &.30 &.49 &.35 &.41 &.50 &.38 &.43 &.37 &.27  &.31 &.45 &.21 &.29 &.48 &.28 &.35 &.52 &.32 &.39\\					
			&non-hate 	&.96 &.97 &.97 &.95 &.99 &.97 &.96 &.98 &.97 &.96 &.98 &.97 &.96 &.97  &.96 &.95 &.98 &.97 &.96 &.98 &.97 &.96 &.98 &.97\\\hline
			
			\multirow{2}{*}{RM}
			&hate 	    &.63 &.60 &.61 &.73 &.69 &.71 &.64 &.75 &.69 &.74 &.65 &.69 &.63 &.56 &.60 &.71 &.65 &.68 &.72 &.60 &.66 &.71 &.64 &.67\\					
			&non-hate 	&.92 &.93 &.92 &.94 &.95 &.94 &.95 &.91 &.93 &.93 &.95 &.94 &.91 &.93 &.92 &.93 &.95 &.94 &.92 &.95 &.94 &.93 &.95 &.94\\
				\hline

    \end{tabular}
		\caption{Full results obtained by the CNN+GRU and CNN+sCNN models.}
		\label{tab_full_results_dnnplus}
\end{table}




% 	WZ-L		&81.5	&81.0	&80.8	&80.7	&81.4	&80.5	&73.6	&74.2\\ 
%				\hline
%	WZ-S.amt	&90.2	&91.6	&89.4	&91.6	&90.1	&91.4	&86.2	&86.7\\ 
%				\hline 
%	WZ-S.exp	&90.4	&91.8	&90.1	&91.2	&90.4	&89.8	&89.1	&90.4\\ 
%				\hline 
%	WZ-S.gb		&91.1	&92.4	&90.0	&91.7	&90.9	&91.0	&86.2	&86.7\\ 
%				\hline 
%	WZ-LS   	&81.4	&82.1	&79.4	&81.3	&81.7	&81.3	&71.6	&72.5\\ 
%				\hline
%	DT			&93.9	&94.2	&92.3	&93.6	&93.1	&94.4	&86.6	&89.4\\ 
%				\hline
%	RM			&90.3	&91.8	&90.0	&90.6	&90.1	&90.1	&85.7	&88.7\\ 




==> tables/tab_full_results_dnnplus_before-double-pooling.tex <==
\begin{table*}[thb]
    \centering
    	\caption{Full results obtained by the CNN+GRU and CNN+sCNN models.}
    \begin{tabular}{p{1cm}|p{1.0cm}|p{0.2cm}p{0.2cm}p{0.2cm}|p{0.2cm}p{0.2cm}p{0.2cm}|p{0.2cm}p{0.2cm}p{0.2cm}|p{.2cm}p{0.2cm}p{0.2cm}|p{0.2cm}p{0.2cm}p{0.2cm}|p{.2cm}p{0.2cm}p{0.2cm}}
%    \begin{tabular}{c| c| c |c| c| c}
        \hline
        	\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Dataset and classes}}}&  
        	\multicolumn{9}{c|}{\textbf{CNN+sCNN}}& 
        	\multicolumn{9}{c}{\textbf{CNN+GRU}}\\\cline{3-20}
        	\multicolumn{2}{c|}{}& \multicolumn{3}{c|}{e.w2v} & \multicolumn{3}{c|}{e.twt} & \multicolumn{3}{c|}{e.glv} & \multicolumn{3}{c|}{e.w2v} & \multicolumn{3}{c|}{e.twt} & \multicolumn{3}{c}{e.glv}\\\hline
        	
        	\multirow{4}{*}{WZ-S.amt}& 	& P &R &F & P &R &F & P &R &F & P &R &F & P &R &F & P &R &F\\\cline{2-20}
        			&racism 	&.45 &.22 &.29 &.43 &.26 &.32 &.36 &.21 &.26 &.44 &.14 &.21 &.44 &.15 &.22 &.48 &.18 &.26\\
        			&sexism 	&.84 &.78 &.81 &.80 &.79 &.79 &.81 &.81 &.81 &.84 &.75 &.80 &.86 &.74 &.79 &.83 &.77 &.80\\        			
        			&non-hate 	&.94 &.97 &.95 &.94 &.96 &.95 &.95 &.96 &.95 &.93 &.97 &.95 &.93 &.97 &.95 &.94 &.97 &.95\\\hline
    		
    		\multirow{3}{*}{WZ-S.exp}
    		&racism 	&.60 &.57 &.58 &.59  &.67 &.63 &.52 &.64 &.57 &.52 &.48 &.50 &.58 &.26 &.36 &.50 &.26 &.34\\
    		&sexism 	&.72 &.65 &.68 &.68  &.76 &.72 &.67 &.74 &.70 &.67 &.64 &.65 &.75 &.60 &.67 &.74 &.61 &.67\\    		
    		&non-hate 	&.93 &.95 &.96 &.96  &.95 &.95 &.96 &.95 &.95 &.94 &.96 &.95 &.93 &.97 &.95 &.94 &.97 &.95\\\hline
			
			\multirow{3}{*}{WZ-S.gb}
			&racism 	&.55 &.53 &.54 &.53 &.63 &.58 &.50 &.52 &.51 &.54 &.47 &.50 &.62 &.38 &.47 &.66 &.34 &.45\\
			&sexism 	&.82 &.73 &.77 &.78 &.79 &.79 &.78 &.80 &.79 &.79 &.76 &.77 &.82 &.74 &.78 &.81 &.75 &.78\\			
			&non-hate 	&.94 &.97 &.96 &.96 &.96 &.96 &.96 &.96 &.96 &.95 &.96 &.96 &.95 &.97 &.96 &.95 &.97 &.96\\\hline
			
			\multirow{3}{*}{WZ.pj}
			&racism 	&.72 &.73 &.73 &.64 &.86 &.74 &.69 &.80 &.74 &.73 &.67 &.70 &.73 &.72 &.72 &.72 &.76 &.74\\
			&sexism 	&.75 &.64 &.69 &.69 &.71 &.70 &.70 &.67 &.68 &.76 &.61 &.68 &.75 &.62 &.68 &.75 &.62 &.68\\			
			&non-hate   &.86 &.90 &.88 &.89 &.84 &.86 &.87 &.87 &.87 &.85 &.91 &.88 &.85 &.90 &.88 &.86 &.90 &.88\\\hline
			
			\multirow{3}{*}{WZ}
			&racism 	&.73 &.74 &.74 &.64 &.87 &.74  &.69 &.84 &.76 &.75 &.70 &.73 &.74 &.74 &.74&.74 &.72 &.73\\
			&sexism 	&.79 &.59 &.68 &.73 &.63 &.68  &.73 &.63 &.68 &.76 &.62 &.68 &.76 &.59 &.67&.78 &.57 &.66\\			
			&non-hate 	&.85 &.91 &.88 &.87 &.86 &.87  &.87 &.87 &.87 &.85 &.91 &.88 &.85 &.90 &.88 &.84 &.91 &.88\\\hline
			
			\multirow{2}{*}{DT}
			&hate 	    &.51 &.21 &.30 &.49 &.35 &.41 &.50 &.38 &.43 &.45 &.21 &.29 &.48 &.28 &.35 &.52 &.32 &.39\\					
			&non-hate 	&.95 &.99 &.97 &.96 &.98 &.97 &.96 &.98 &.97 &.95 &.98 &.97 &.96 &.98 &.97 &.96 &.98 &.97\\\hline
			
			\multirow{2}{*}{RM}
			&hate 	    &.73 &.69 &.71 &.64 &.75 &.69 &.74 &.65 &.69 &.71 &.65 &.68 &.72 &.60 &.66 &.71 &.64 &.67\\					
			&non-hate 	&.94 &.95 &.94 &.95 &.91 &.93 &.93 &.95 &.94 &.93 &.95 &.94 &.92 &.95 &.94 &.93 &.95 &.94\\
				\hline

    \end{tabular}
	
		\label{tab_full_results_dnnplus}
\end{table*}




% 	WZ-L		&81.5	&81.0	&80.8	&80.7	&81.4	&80.5	&73.6	&74.2\\ 
%				\hline
%	WZ-S.amt	&90.2	&91.6	&89.4	&91.6	&90.1	&91.4	&86.2	&86.7\\ 
%				\hline 
%	WZ-S.exp	&90.4	&91.8	&90.1	&91.2	&90.4	&89.8	&89.1	&90.4\\ 
%				\hline 
%	WZ-S.gb		&91.1	&92.4	&90.0	&91.7	&90.9	&91.0	&86.2	&86.7\\ 
%				\hline 
%	WZ-LS   	&81.4	&82.1	&79.4	&81.3	&81.7	&81.3	&71.6	&72.5\\ 
%				\hline
%	DT			&93.9	&94.2	&92.3	&93.6	&93.1	&94.4	&86.6	&89.4\\ 
%				\hline
%	RM			&90.3	&91.8	&90.0	&90.6	&90.1	&90.1	&85.7	&88.7\\ 




==> tables/tab_ratios.tex <==
\begin{table}[thb]
    \centering
%    \begin{tabular}{p{1.3cm}|c|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{3cm}}
    \begin{tabular}{c| c| c |c| c| c}
        \hline
        	& \textbf{Racism}	& \textbf{Sexism} 	& \textbf{Both}	&\textbf{Non-hate}	&\textbf{Hate}\\\hline
    
	WZ-S.amt	&0.15	&0.29	&0.10	&0.65	&-		\\ 
				\hline 
	WZ-S.exp	&0.21	&0.26	&0.16	&0.72	&-	\\ 
				\hline 
	WZ-S.gb		&0.20	&0.28	&0.14	&0.70	&-	\\ 
				\hline 
  	WZ.pj		&0.15	&0.27	&0.10	&0.55	&-	\\ 
				\hline
	WZ	   		&0.16	&0.27	&-		&0.55	&-\\ 				
				\hline
	DT			&-		&-		&-		&0.82	&0.15	\\ 
				\hline
	RM			&-		&-		&-		&0.78	&0.27\\ 
	
				\hline

    \end{tabular}
		\caption{Analysis of Uwords-2-Class (U2C) ratios.}
		\label{table_ratios}
\end{table}




% 	WZ-L		&81.5	&81.0	&80.8	&80.7	&81.4	&80.5	&73.6	&74.2\\ 
%				\hline
%	WZ-S.amt	&90.2	&91.6	&89.4	&91.6	&90.1	&91.4	&86.2	&86.7\\ 
%				\hline 
%	WZ-S.exp	&90.4	&91.8	&90.1	&91.2	&90.4	&89.8	&89.1	&90.4\\ 
%				\hline 
%	WZ-S.gb		&91.1	&92.4	&90.0	&91.7	&90.9	&91.0	&86.2	&86.7\\ 
%				\hline 
%	WZ-LS   	&81.4	&82.1	&79.4	&81.3	&81.7	&81.3	&71.6	&72.5\\ 
%				\hline
%	DT			&93.9	&94.2	&92.3	&93.6	&93.1	&94.4	&86.6	&89.4\\ 
%				\hline
%	RM			&90.3	&91.8	&90.0	&90.6	&90.1	&90.1	&85.7	&88.7\\ 




==> tables/tab_ratios_both.tex <==
\begin{table*}[thb]
    \centering
%    \begin{tabular}{p{1.3cm}|c|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{3cm}}
    \begin{tabular}{c|c c| c c |c c| cc| cc}
        \hline
        	& \multicolumn{2}{c|}{\textbf{Racism}}	& \multicolumn{2}{c|}{\textbf{Sexism}} 	& \multicolumn{2}{c|}{\textbf{Both}}	&\multicolumn{2}{c|}{\textbf{Non-hate}}	&\multicolumn{2}{c}{\textbf{Hate}}\\
  				&I2U	&U2C	&I2U	&U2C	&I2U	&U2C	&I2U	&U2C	&I2U	&U2C\\\cline{2-11}
    
	WZ-S.amt	&0.17	&0.15	&0.43	&0.29	&0.09	&0.10	&0.95	&0.65	&-		&-\\ 
				\hline 
	WZ-S.exp	&0.16	&0.21	&0.38	&0.26	&0.13	&0.16	&0.98	&0.72	&-	&-	\\ 
				\hline 
	WZ-S.gb		&0.17	&0.20	&0.41	&0.28	&0.13	&0.14	&0.97	&0.70	&-	&-	\\ 
				\hline 
  	WZ.pj		&0.71	&0.15	&0.76	&0.27	&0.13	&0.10	&1.4	&0.55	&-	&-	\\ 
				\hline
	WZ	   		&0.74	&0.16	&0.71	&0.27	&-		&-		&1.4	&0.55	&-	&-	\\ 				
				\hline
	DT			&-		&-		&-		&-		&-		&-		&1.6	&0.82	&0.49	&0.15	\\ 
				\hline
	RM			&-		&-		&-		&-		&-		&-		&0.48	&0.78	&0.32	&0.27\\ 
	
				\hline

    \end{tabular}
		\caption{Analysis of Instance-2-Uwords (I2U) and Uwords-2-Class (U2C) ratios.}
		\label{table_ratios}
\end{table*}




% 	WZ-L		&81.5	&81.0	&80.8	&80.7	&81.4	&80.5	&73.6	&74.2\\ 
%				\hline
%	WZ-S.amt	&90.2	&91.6	&89.4	&91.6	&90.1	&91.4	&86.2	&86.7\\ 
%				\hline 
%	WZ-S.exp	&90.4	&91.8	&90.1	&91.2	&90.4	&89.8	&89.1	&90.4\\ 
%				\hline 
%	WZ-S.gb		&91.1	&92.4	&90.0	&91.7	&90.9	&91.0	&86.2	&86.7\\ 
%				\hline 
%	WZ-LS   	&81.4	&82.1	&79.4	&81.3	&81.7	&81.3	&71.6	&72.5\\ 
%				\hline
%	DT			&93.9	&94.2	&92.3	&93.6	&93.1	&94.4	&86.6	&89.4\\ 
%				\hline
%	RM			&90.3	&91.8	&90.0	&90.6	&90.1	&90.1	&85.7	&88.7\\ 




==> tables/tab_result.tex <==
\begin{table}[thb]
    \centering
%    \begin{tabular}{p{1.3cm}|c|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{3cm}}
    \begin{tabular}{c|cc c c |c | c l}
        \hline
        \multirow{2}{*}{\textbf{Dataset}} 	&\multirow{2}{*}{\textbf{SVM}}	&\multirow{2}{*}{\textbf{SVM+}}		& \multirow{2}{*}{\textbf{CNN}}	& \textbf{CNN+}	& \textbf{CNN+} & \multicolumn{2}{c}{\multirow{2}{*}{\textbf{State of the art}}}\\
      	&	&	 & &\textbf{GRU}\textsubscript{B}	&\textbf{GRU}	& & \\
				\hline
  	WZ-L		&0.74	&0.74	&0.80	&0.81	&\textbf{0.82}	&0.74	&Waseem \cite{Waseem2016a}, best F1\\ 
				\hline	
	WZ-S.amt	&0.86	&0.87	&0.91	&\textbf{0.92}	&\textbf{0.92}	&0.84	&Waseem \cite{Waseem2016b}, `Best' features\\ 
				\hline 
	WZ-S.exp	&0.89	&0.90	&0.90	&0.91	&\textbf{0.92}	&0.91	&Waseem \cite{Waseem2016b}, `Best' features\\ 
				\hline 
	WZ-S.gb		&0.86	&0.87	&0.91	&0.92	&\textbf{0.93}	&0.90	&Gamback \cite{Gamback2017}, best F1\\ 
				\hline 
	\multirow{3}{*}{WZ-LS}   	&\multirow{3}{*}{0.72}	&\multirow{3}{*}{0.73}	&\multirow{3}{*}{0.81}	&\multirow{3}{*}{0.81}	&\multirow{3}{*}{0.82}	&0.82	&Park \cite{Park2017}, WordCNN	\\ 
				&				&		&		&		&		&0.81		&Park \cite{Park2017}, CharacterCNN\\
				&				&		&		&		&		&\textbf{0.83}		&Park \cite{Park2017}, HybridCNN\\							
				\hline
	DT			&0.87	&0.89	&\textbf{0.94}	&\textbf{0.94}	&\textbf{0.94}	&0.87	&SVM, Davidson \cite{Davidson2017}\\ 
				\hline
	RM			&0.86	&0.89	&0.90	&0.91	&\textbf{0.92}	&0.86	&SVM, Davidson \cite{Davidson2017}\\ 
				\hline

    \end{tabular}
		\caption{F1 result of the proposed method against baselines and state of the art. The best figures are highlighted in \textbf{bold}.}
		\label{tab_result}
\end{table}




% 	WZ-L		&81.5	&81.0	&80.8	&80.7	&81.4	&80.5	&73.6	&74.2\\ 
%				\hline
%	WZ-S.amt	&90.2	&91.6	&89.4	&91.6	&90.1	&91.4	&86.2	&86.7\\ 
%				\hline 
%	WZ-S.exp	&90.4	&91.8	&90.1	&91.2	&90.4	&89.8	&89.1	&90.4\\ 
%				\hline 
%	WZ-S.gb		&91.1	&92.4	&90.0	&91.7	&90.9	&91.0	&86.2	&86.7\\ 
%				\hline 
%	WZ-LS   	&81.4	&82.1	&79.4	&81.3	&81.7	&81.3	&71.6	&72.5\\ 
%				\hline
%	DT			&93.9	&94.2	&92.3	&93.6	&93.1	&94.4	&86.6	&89.4\\ 
%				\hline
%	RM			&90.3	&91.8	&90.0	&90.6	&90.1	&90.1	&85.7	&88.7\\ 




==> tables/tab_result_soa.tex <==
\begin{table}[thb]
    \centering
%    \begin{tabular}{p{1.3cm}|c|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{3cm}}
    \begin{tabular}{c|cc|cl}
        \hline
        \multirow{2}{*}{\textbf{Dataset}} 		& \multicolumn{2}{c|}{\textbf{CNN+GRU}} 	& \multicolumn{2}{c}{\textbf{State of the art}} 	\\\cline{2-5}
        						& e.lrn	&e.ggl	&score 	&source\\
				\hline
 
 	WZ-L		&81.5	&81.0	&73.9	&Waseem et al., best F1 in \cite{Waseem2016a}	\\ 
				\hline
	WZ-S.amt	&90.2	&91.6	&83.9	&Waseem et al., the 'Best' feature set in \cite{Waseem2016b}	\\ 
				\hline 
	WZ-S.exp	&90.4	&91.8	&91.2	&Waseem et al., the 'Best' feature set in \cite{Waseem2016b}	\\ 
				\hline 
	WZ-S.gb		&91.1	&92.4	&90.0	&Gamback et al., best F1 in \cite{Gamback2017}	\\ 
				\hline 
	\multirow{3}{*}{WZ-LS}   	&\multirow{3}{*}{81.4}	&\multirow{3}{*}{82.1}	&81.6	&WordCNN in Park et al. \cite{Park2017}	\\ 
	   	&	&	&81.1	&CharacterCNN in Park et al. \cite{Park2017}	\\ 
	  	&	&	&82.7	&HybridCNN in Park et al. \cite{Park2017}	\\ 
				\hline
	DT			&93.9	&94.2	&86.5	&SVM baseline as Davidson et al. \cite{Davidson2017}	\\ 
				\hline
	RM			&90.3	&91.8	&85.7	&SVM baseline as Davidson et al. \cite{Davidson2017}	\\ 
				\hline
    \end{tabular}
		\caption{F1 result of the proposed method against state of the art. The best figures are highlighted in \textbf{bold}.}
		\label{tab_result_soa}
\end{table}




==> tables/tab_result_soa_before-correction.tex <==
\begin{table}[thb]
    \centering
%    \begin{tabular}{p{1.3cm}|c|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{3cm}}
    \begin{tabular}{c|cc|cl}
        \hline
        \multirow{2}{*}{\textbf{Dataset}} 		& \multicolumn{2}{c|}{\textbf{CNN+GRU}} 	& \multicolumn{2}{c}{\textbf{State of the art}} 	\\\cline{2-5}
        						& e.lrn	&e.ggl	&score 	&source\\
				\hline
 
 	WZ-L		&81.5	&81.0	&73.9	&Waseem et al., best F1 in \cite{Waseem2016a}	\\ 
				\hline
	WZ-S.amt	&90.2	&91.6	&83.9	&Waseem et al., the 'Best' feature set in \cite{Waseem2016b}	\\ 
				\hline 
	WZ-S.exp	&90.4	&91.8	&91.2	&Waseem et al., the 'Best' feature set in \cite{Waseem2016b}	\\ 
				\hline 
	WZ-S.gb		&91.1	&92.4	&90.0	&Gamback et al., best F1 in \cite{Gamback2017}	\\ 
				\hline 
	\multirow{3}{*}{WZ-LS}   	&\multirow{3}{*}{81.4}	&\multirow{3}{*}{82.1}	&81.6	&WordCNN in Park et al. \cite{Park2017}	\\ 
	   	&	&	&81.1	&CharacterCNN in Park et al. \cite{Park2017}	\\ 
	  	&	&	&82.7	&HybridCNN in Park et al. \cite{Park2017}	\\ 
				\hline
	DT			&93.9	&94.2	&86.5	&SVM baseline as Davidson et al. \cite{Davidson2017}	\\ 
				\hline
	RM			&90.3	&91.8	&85.7	&SVM baseline as Davidson et al. \cite{Davidson2017}	\\ 
				\hline
    \end{tabular}
		\caption{F1 result of the proposed method against state of the art. The best figures are highlighted in \textbf{bold}.}
		\label{tab_result_soa}
\end{table}




==> tables/tab_results_before-correction.tex <==
\begin{table*}[thb]
    \centering
    \caption{Micro v.s. macro F1 results of different methods (using the Word2Vec embeddings). The best results on each row are highlighted in \textbf{bold}. Numbers within (brackets) indicate the improvement in F1 compared to the \textit{best result} by any of the three state of the art methods.}
    \begin{tabular}{c | l | c c c| c c c c}
%    \begin{tabular}{c| c| c |c| c| c}
        \hline
        	\textbf{Dataset} &\textbf{Measure}& \textbf{SVM}	& \textbf{GB}& 
        	\textbf{PK}	&\multicolumn{2}{c}{\textbf{CNN+sCNN}}	&\multicolumn{2}{c}{\textbf{CNN+GRU}}\\\hline        
        	
        	\multirow{3}{*}{WZ-S.amt}
        			&micro F1 	&0.81 &\textbf{0.92} &\textbf{0.92} &\textbf{0.92} &(-) &\textbf{0.92} &(-)\\
        			&macro F1 	&0.59 &0.63 &0.64 &\textbf{0.68} &(+0.04) &0.65 &(+0.01)\\        			
        			&macro F1, hate 	&0.45 &0.48 &0.49 &\textbf{0.55} &(+0.06) &0.51 &(+0.02) \\\hline
    		
    		\multirow{3}{*}{WZ-S.exp}
    		&micro F1 	&0.82 &0.91 &0.91 &\textbf{0.92} &(+0.01) &\textbf{0.92} &(+0.01) \\
    		&macro F1 	&0.58 &0.69 &0.69  &\textbf{0.74} &(+0.05) &0.70 &(+0.01) \\    		
    		&macro F1, hate &0.42 &0.57 &0.56  &\textbf{0.63} &(+0.06) &0.58 &(+0.01) \\\hline
			
			\multirow{3}{*}{WZ-S.gb}
			&micro F1 &0.83 &0.92 &0.92 &\textbf{0.93} &(+0.01) &\textbf{0.93} &(+0.01) \\
			&macro F1 &0.64 &0.70 &0.70 &\textbf{0.76} &(+0.06) &0.74 &(+0.04) \\			
			&macro F1, hate 	&0.51 &0.57 &0.57 &\textbf{0.66} &(+0.09) &0.64 &(+0.07) \\\hline
			
			\multirow{3}{*}{WZ.pj}
			&micro F1 &0.72 &0.82 &0.82 &\textbf{0.83} &(+0.01) &\textbf{0.83} &(+0.01) \\
			&macro F1 &0.66 &0.74 &0.75 &\textbf{0.77} &(+0.02) &0.75 &(-) \\			
			&macro F1, hate 	&0.59 &0.68 &0.69 &\textbf{0.71} &(+0.02) &0.69 &(-) \\\hline
			
			\multirow{3}{*}{WZ}
			&micro F1 &0.72 &0.82 &0.82 &\textbf{0.83} &(+0.01) &\textbf{0.83} &(+0.01) \\
			&macro F1 &0.65 &0.75 &0.75 &\textbf{0.77} &(+0.02) &0.76 &(+0.01) \\			
			&macro F1, hate &0.58 &0.70 &0.69 &\textbf{0.71} &(+0.01) &\textbf{0.71} &(+0.01) \\\hline
			
			\multirow{3}{*}{DT}
			&micro F1   &0.79 &\textbf{0.94} &\textbf{0.94} &\textbf{0.94} &(-) &\textbf{0.94} &(-) \\					
			&macro F1   &0.56 &0.61 &0.60 &\textbf{0.64} &(+0.03) &0.63 &(+0.02) \\
			&macro F1, hate 	&0.23 &0.25 &0.23 &\textbf{0.30} &(+0.05) &0.29 &(+0.04) \\\hline
			
			\multirow{3}{*}{RM}
			&micro F1   &0.79 &0.90  &0.90 &\textbf{0.91} &(+0.01) &0.90 &(-) \\					
			&macro F1 	&0.72 &0.80  &0.81 &\textbf{0.83} &(+0.02) &0.81 &(+0.01) \\
			&macro F1, hate 	&0.58 &0.67 &.68 &\textbf{0.71} &(+0.03) &0.68 &(-) \\
				\hline

    \end{tabular}
		
		\label{tab_results}
\end{table*}




% 	WZ-L		&81.5	&81.0	&80.8	&80.7	&81.4	&80.5	&73.6	&74.2\\ 
%				\hline
%	WZ-S.amt	&90.2	&91.6	&89.4	&91.6	&90.1	&91.4	&86.2	&86.7\\ 
%				\hline 
%	WZ-S.exp	&90.4	&91.8	&90.1	&91.2	&90.4	&89.8	&89.1	&90.4\\ 
%				\hline 
%	WZ-S.gb		&91.1	&92.4	&90.0	&91.7	&90.9	&91.0	&86.2	&86.7\\ 
%				\hline 
%	WZ-LS   	&81.4	&82.1	&79.4	&81.3	&81.7	&81.3	&71.6	&72.5\\ 
%				\hline
%	DT			&93.9	&94.2	&92.3	&93.6	&93.1	&94.4	&86.6	&89.4\\ 
%				\hline
%	RM			&90.3	&91.8	&90.0	&90.6	&90.1	&90.1	&85.7	&88.7\\ 




==> tables/tab_results_per_class_before-correction.tex <==
\begin{table*}[thb]
    \centering
    \caption{F1 results of different models for each class (using the Word2Vec embeddings). The best results on each row are highlighted in \textbf{bold}. Numbers within (brackets) indicate the improvement in F1 compared to the \textit{best results} from any of the three state of the art methods.}
    \begin{tabular}{c | c | c c c| c c c c}
%    \begin{tabular}{c| c| c |c| c| c}
        \hline
        	\textbf{Dataset} &\textbf{Class}& \textbf{SVM}	& \textbf{GB}& 
        	\textbf{PK}	&\multicolumn{2}{c}{\textbf{CNN+sCNN}}	&\multicolumn{2}{c}{\textbf{CNN+GRU}}\\\hline        
        	
        	\multirow{3}{*}{WZ-S.amt}
        			&racism 	&0.22 &0.15 &0.18 &\textbf{0.29} &(+0.07) &0.21 &(-0.01)\\
        			&sexism 	&0.68 &0.80 &0.80 &\textbf{0.81} &(+0.01) &0.80 &(-)\\        			
        			&non-hate 	&0.88 &\textbf{0.95} &\textbf{0.95} &\textbf{0.95} &(-) &\textbf{0.95} &(-) \\\hline
    		
    		\multirow{3}{*}{WZ-S.exp}
    		&racism 	&0.26 &0.49 &0.46  &\textbf{0.58} &(+0.09) &0.50 &(+0.01) \\
    		&sexism 	&0.58 &0.65 &0.65  &\textbf{0.68} &(+0.03) &0.65 &(-) \\    		
    		&non-hate   &0.89 &0.95 &\textbf{0.97}  &0.96 &(-0.01) &0.95 &(-0.02) \\\hline
			
			\multirow{3}{*}{WZ-S.gb}
			&racism 	&0.38 &0.38 &0.37 &\textbf{0.54} &(+0.16) &0.50 &(+0.12) \\
			&sexism 	&0.64 &0.75 &0.76 &\textbf{0.77} &(+0.02) &0.77 &(+0.01) \\			
			&non-hate 	&0.90 &\textbf{0.96} &\textbf{0.96} &\textbf{0.96} &(-) &\textbf{0.96} &(-) \\\hline
			
			\multirow{3}{*}{WZ.pj}
			&racism 	&0.60 &0.69 &0.70 &\textbf{0.73} &(+0.03) &0.70 &(-) \\
			&sexism 	&0.58 &0.67 &0.68 &\textbf{0.69} &(+0.01) &0.68 &(-) \\			
			&non-hate 	&0.80 &\textbf{0.88} &\textbf{0.88} &\textbf{0.88} &(-) &\textbf{0.88} &(-) \\\hline
			
			\multirow{3}{*}{WZ}
			&racism 	&0.59 &0.72 &0.71 &\textbf{0.74} &(+0.02) &0.73 &(+0.01) \\
			&sexism 	&0.57 &0.67 &0.67 &\textbf{0.68} &(+0.01) &\textbf{0.68} &(+0.01) \\			
			&non-hate   &0.79 &\textbf{0.88} &\textbf{0.88} &\textbf{0.88} &(-) &\textbf{0.88} &(-) \\\hline
			
			\multirow{2}{*}{DT}
			&hate 	    &0.23 &0.25 &0.23 &\textbf{0.30} &(+0.05) &0.29 &(+0.04) \\					
			&non-hate 	&0.88 &\textbf{0.97} &\textbf{0.97} &\textbf{0.97} &(-) &\textbf{0.97} &(-) \\\hline
			
			\multirow{2}{*}{RM}
			&hate 	    &0.58 &0.67  &0.68 &\textbf{0.71} &(+.03) &0.68 &(-) \\					
			&non-hate 	&0.86 &\textbf{0.94}  &\textbf{0.94} &\textbf{0.94} &(-) &\textbf{0.94} &(-) \\
				\hline

    \end{tabular}
		
		\label{tab_results_per_class}
\end{table*}




% 	WZ-L		&81.5	&81.0	&80.8	&80.7	&81.4	&80.5	&73.6	&74.2\\ 
%				\hline
%	WZ-S.amt	&90.2	&91.6	&89.4	&91.6	&90.1	&91.4	&86.2	&86.7\\ 
%				\hline 
%	WZ-S.exp	&90.4	&91.8	&90.1	&91.2	&90.4	&89.8	&89.1	&90.4\\ 
%				\hline 
%	WZ-S.gb		&91.1	&92.4	&90.0	&91.7	&90.9	&91.0	&86.2	&86.7\\ 
%				\hline 
%	WZ-LS   	&81.4	&82.1	&79.4	&81.3	&81.7	&81.3	&71.6	&72.5\\ 
%				\hline
%	DT			&93.9	&94.2	&92.3	&93.6	&93.1	&94.4	&86.6	&89.4\\ 
%				\hline
%	RM			&90.3	&91.8	&90.0	&90.6	&90.1	&90.1	&85.7	&88.7\\ 



